How Costly is Noise? Data and Disparities in Consumer Credit

We show that lenders face more uncertainty when assessing default risk of historically under-served groups in US credit markets and that this information disparity is a quantitatively important driver of inefficient and unequal credit market outcomes. We first document that widely used credit scores are statistically noisier indicators of default risk for historically under-served groups. This noise emerges primarily through the explanatory power of the underlying credit report data (e.g., thin credit files), not through issues with model fit (e.g., the inability to include protected class in the scoring model). Estimating a structural model of lending with heterogeneity in information, we quantify the gains from addressing these information disparities for the US mortgage market. We find that equalizing the precision of credit scores can reduce disparities in approval rates and in credit misallocation for disadvantaged groups by approximately half.

==> Tables/tb_AUCDifferences_ByCreditReportContent.tex <==
%----- ----- ----- ----- ----- ----- -----%
% Table Name :
% Source     :
% Version    :
% Date       :
% Author     :
% Description:
%----- ----- ----- ----- ----- ----- -----%

\begin{tabular}{lccccccc}\toprule
AUC & Minority=0 & Minority=1 & $\Delta$& & Low income=0 & Low income=1 &$\Delta$ \\\midrule
No Mortgage & 0.827 & 0.793 & 0.034 & & 0.825 & 0.799 & 0.026 \\
& (0.001) & (0.001) & & & (0.001) & (0.001) & \\
1+ Mortgage & 0.819 & 0.800 & 0.019 & & 0.815 & 0.802 & 0.013 \\
& (0.001) & (0.002) & & & (0.001) & (0.002) & \\\midrule
No Auto Loan & 0.844 & 0.798 & 0.046 & & 0.833 & 0.812 & 0.021 \\
& (0.001) & (0.003) & & & (0.002) & (0.002) & \\
1+ Auto Loan & 0.832 & 0.811 & 0.021 & & 0.820 & 0.799 & 0.021 \\
& (0.001) & (0.001) & & & (0.001) & (0.001) & \\\midrule
No Bankcard & 0.794 & 0.738 & 0.056 & & 0.806 & 0.757 & 0.049 \\
& (0.001) & (0.003)  & & & (0.002) & (0.002)  & \\
1+ Bankcard & 0.816 & 0.790 & 0.026 & & 0.806 & 0.786 & 0.020 \\
& (0.001) & (0.001)  & & & (0.001) & (0.001)  & \\\midrule
No Account & 0.437 & 0.402 & 0.035 & & 0.702 & 0.603 & 0.099 \\
& (0.011) & (0.011) & & & (0.030) & (0.035) & \\
1+ Account & 0.835 & 0.812 & 0.023 & & 0.823 & 0.803 & 0.020 \\
& (0.001) & (0.001)& & & (0.001) & (0.001) & \\\midrule
No History & 0.771 & 0.696 & 0.075 & & no obs & 0.722 & . \\
& (0.051) & 0.093 & & & & (0.054) & \\
1+ History & 0.835 & 0.812 & 0.023 & & 0.823 & 0.803 & 0.020 \\
& (0.001) & (0.001) & & & (0.001) & (0.001)& \\\bottomrule
\end{tabular}

==> Tables/tb_ConfusionMatrices_DefaultMeasures.tex <==
%----- ----- ----- ----- ----- ----- -----%
% Table Name :
% Source     :
% Version    :
% Date       :
% Author     :
% Description:
%----- ----- ----- ----- ----- ----- -----%
\begin{tabular}{ccccccc}\toprule
& \multicolumn{2}{c}{ Mortgage delinquency } & &  & \multicolumn{2}{c}{ Mortgage  delinquency } \\
Any delinquency & 0 & 1 && At least 60 days & 0 & 1 \\
0 & 15,281,777 & 0 &&  0 & 16,684,878 & 325,570 \\
1 & 2,728,975 & 1,102,001 & & 1 & 1,325,874 & 776,464 \\
& & & & &\\
\emph{Precision} & 0.29 & & & \emph{Precision} & 0.37 & \\
\emph{Recall} & 1.00 & & & \emph{Recall} & 0.70 & \\
\emph{Accuracy} & 0.86 & & &\emph{Accuracy} & 0.91 & \\ \midrule
& & & & &\\
& \multicolumn{2}{c}{ Mortgage delinquency } &  && \multicolumn{2}{c}{ Mortgage delinquency } \\
At least 90 days & 0 & 1 && At least 120 days & 0 & 1 \\
0 & 16,946,972 & 410,921 && 0 & 17,067,672 & 458,210 \\
1 & 1,063,780 & 691,113 && 1 & 943,080 & 643,824 \\
& & & & &\\
\emph{Precision} & 0.39 & &&\emph{Precision} & 0.41 & \\
\emph{Recall} & 0.63 & && \emph{Recall} & 0.58 & \\
\emph{Accuracy} & 0.92 & && \emph{Accuracy} & 0.93 & \\ \midrule
& & & & &\\
& \multicolumn{2}{c}{ Mortgage  delinquency } && Memo: & \multicolumn{2}{c}{ Actual default } \\
Severe derogatory & 0 & 1 && Predicted default & 0 & 1 \\
0 & 17,207,007 & 558,990 && 0 & TN & FN \\
1 & 803,745 & 543,044 && 1 & FP & TP \\
& & & & &\\
\emph{Precision} & 0.40& && \emph{Precision} & TP/(TP+FP) & \\
\emph{Recall} & 0.49 && & \emph{Recall} & TP/(TP+FN) & \\
\emph{Accuracy} & 0.93 & && \emph{Accuracy} & (TP+TN)/N & \\\bottomrule
\end{tabular}

==> Tables/tb_InformationContent_CreditReportingFiles.tex <==
%----- ----- ----- ----- ----- ----- -----%
% Table Name : Information Concent on Credit Report Files
% Source     :
% - GH: https://github.com/bimetal1896/BlattnerNelson/pull/145
% - DB: https://www.dropbox.com/home/BlattnerNelsonShared/TU/Stylized_facts/Credit_report_info/october2020_jh
% Version    : 1.1
% Date       : 201021
% Author     : 1.0 Laura Blattner
% Author     : 1.1 Jacob Hartwig 
% Note       : The table shows regression results in the sample of mortgage applicants. We regress the variable of interest on a constant and two dummies indicating either minority or low income status. Standard errors are shown in parentheses.
%----- ----- ----- ----- ----- ----- -----%

% Variables:
% C1: trdcnt     = Number of accounts
% C2: trdmof     = Number of months on file
% C3: less1_card = 1 credit card or less
% C4: bkopenth   = Number of bank cards
% C5: auttrds    = Number of auto trades

\begin{tabular}{lccccc} \toprule
           & Number of accounts & Number of months on file & 1 credit card or less & Number of bank cards & Number of auto trades \\ \midrule
&                    &                          &                       &                      &                       \\
Constant   & 22.51***           & 259.8***                 & 0.310***              & 3.008***             & 2.965***             \\
           & (0.151)            & (1.411)                  & (0.00322)             & (0.0198)             & (0.00949)            \\
Minority   & -0.161             & -9.490***                & 0.0691***             & -0.184***            & -0.160***            \\
           & (0.175)            & (1.630)                  & (0.00372)             & (0.0229)             & (0.0110)             \\
Low income & -9.973***          & -67.07***                & 0.300***              & -1.491***            & -1.368***            \\
           & (0.175)            & (1.630)                  & (0.00372)             & (0.0229)             & (0.0110)             \\
           &                    &                          &                       &                      &                      \\
N          & 44,720,376         & 44,720,376               & 44,720,376            & 44,720,376           & 44,720,376           \\ \bottomrule
%           &                    &                          &                       &                      &                       \\
\end{tabular}

==> Tables/tb_ModelEstimation_ModelMoments.tex <==
%----- ----- ----- ----- ----- ----- -----%
% Table Name :
% Source     :
% Version    : TO BE UPDATED
% Date       : 11/18/2020
% Author     : Pranav Garg
% Description:
%----- ----- ----- ----- ----- ----- -----%
    \begin{tabular}{lcccc} \toprule
     & \multicolumn{2}{c}{{Income}}   & \multicolumn{2}{c}{{Minority}} \\
        & High & Low  & Maj. & Min.  \\\toprule
    Approval Rate 	            &	0.551	    &	0.297       &	0.556	    &	0.352	    \\
    Average Default Rate 	    &	0.047	    &	0.101	    &	0.031	    &	0.066	    \\
    Marginal Default Rate 	    &	0.125	    &	0.172	    &	0.096	    &	0.083	    \\
    Avg. Approved Score 	    &	710	        &	610	        &	719	        &	682	        \\
    Avg. Rejected Scores 	    &	634	        &	451	        &	640	        &	558	        \\
    Default vs. Score Slope 	&	-0.00057	&	-0.00081	&	-0.00052	&	-0.00074    \\
    Score vs. Default Slope 	&	-30.999	    &	-52.810	    &	-36.031	    &	-42.088	    \\
    Lender Profit 	            &	0.00	    &	0.00	    &	0.00	    &	0.00	    \\ \bottomrule

    \end{tabular}

==> Tables/tb_auc_composition_lb.tex <==
%----- ----- ----- ----- ----- ----- -----%
% Table Name : Mean AUC with different weighting
% Source     :  
% Version    : 1
% Date       : Feb 17 2021
% Author     : Laura Blattner
% Description:  
%----- ----- ----- ----- ----- ----- -----%

\begin{tabular}{lccrccr}\toprule 
& Low income & Higher income & \multicolumn{1}{c}{$\Delta$} & Minority & Non-minority & \multicolumn{1}{c}{$\Delta$}  \\ 
&  & & & & & \\\midrule
Number of accounts & 0.831 & 0.822 & 0.009 & 0.827 & 0.820 & 0.007 \\
Non-mortgage balance & 0.824 & 0.829 & -0.005 & 0.824 & 0.819 & 0.005 \\
History length & 0.827 & 0.827 & 0.000 & 0.822 & 0.815 & 0.007 \\
Any mortgage & 0.823 & 0.797 & 0.027 & 0.818 & 0.809 & 0.009 \\
Any auto loan & 0.827 & 0.828 & -0.001 & 0.828 & 0.828 & 0.000 \\
Any installment loan & 0.827 & 0.829 & -0.002 & 0.827 & 0.828 & -0.001 \\
Any bankcard & 0.832 & 0.799 & 0.034 & 0.824 & 0.810 & 0.014 \\
Any student loan & 0.827 & 0.827 & 0.000 & 0.827 & 0.827 & 0.000 \\
Utilization & 0.829 & 0.828 & 0.000 & 0.828 & 0.828 & 0.000 \\
Default history & 0.786 & 0.760 & 0.026 & 0.784 & 0.762 & 0.022 \\\bottomrule
\end{tabular}

==> Tables/tb_coefficients_by_group.tex <==
%----- ----- ----- ----- ----- ----- -----%
% Table Name : Model Coefficients by Group 
% Source     : Google shet: ML mortgage model training
% Version    : 1
% Date       : Feb 2021
% Author     : Laura Blattner
% Description: Shows coefficients from 20-variable logit model trained separately by group
%----- ----- ----- ----- ----- ----- -----%


\begin{tabular}{ccccc}\toprule
Logit coefficient & Non-minority & Minority & Higher income & Low income \\\midrule
mvc_cv01_-1.0 & -0.280 & -0.279 & -0.303 & -0.232 \\
out_flag_cv12 & -0.050 & -0.028 & -0.063 & -0.016 \\
cv12 & 0.273 & 0.225 & 0.286 & 0.216 \\
ttl_1m_bi_good & -0.003 & 0.000 & 0.059 & -0.047 \\
out_flag_bankrpth & 0.341 & 0.245 & 0.342 & 0.223 \\
bankrpth & -0.102 & -0.065 & -0.101 & -0.055 \\
mvc_cv04_-6.0 & -0.123 & -0.130 & -0.092 & -0.127 \\
cv13 & 0.257 & 0.188 & 0.292 & 0.165 \\
ttl_3m_bi_badamt & 0.043 & -0.002 & 0.015 & 0.031 \\
ttl_3m_bi_bad & 0.029 & 0.056 & 0.034 & 0.036 \\
bankin12 & 0.120 & 0.159 & 0.127 & 0.132 \\
ttl_3m_bi_good & 0.055 & 0.060 & 0.032 & 0.080 \\
cv01 & -0.527 & -0.418 & -0.562 & -0.404 \\
flag_ft & 0.111 & 0.200 & 0.096 & 0.204 \\
derogpub & -0.036 & 0.004 & -0.043 & -0.004 \\
mvc_cv05_-1.0 & -0.007 & -0.037 & 0.013 & -0.052 \\
mvc_cv05_-6.0 & -0.123 & -0.130 & -0.092 & -0.127 \\
chgof24h & 0.056 & 0.081 & 0.066 & 0.061 \\
mvc_trv21_-1.0 & -0.014 & -0.020 & -0.027 & -0.085 \\
mvc_trv21_-2.0 & 0.088 & 0.107 & 0.040 & 0.114 \\
dpbrec36 & 0.089 & 0.080 & 0.091 & 0.091 \\
outflag_ll_inq_time_since_newest & -0.034 & 0.006 & -0.029 & -0.005 \\\bottomrule
\end{tabular}


==> Tables/tb_noise_bias_data.tex <==
%----- ----- ----- ----- ----- ----- -----%
% Table Name : 
% Source     : 
% Version    :
% Date       : 
% Author     :
% Description: 
%----- ----- ----- ----- ----- ----- -----%


\begin{tabular}{ccccc}
\toprule
& (1) & (2) & (3) & (4) \\
& 90+ days late & 120+ days late & 90+ days late & 120+ days late \\
& & & & \\
Credit score & -0.0104*** & -0.0106*** & -0.0148*** & -0.0150*** \\
& (0.000) & ((0.000) & (0.000) & (0.000)\\
Minority & 0.683*** & 0.695*** & & \\
& (0.000) & (0.000)& & \\
Low income & & & 0.0949*** & 0.106*** \\
& & &(0.000) & (0.000) \\
Constant & 5.266*** & 5.303*** & 8.505*** & 8.534*** \\
&(0.000) & (0.000) & (0.000) & (0.000) \\
& & & & \\
Observations & 16,618,186 & 16,618,186 & 46,869,904 & 46,869,904 \\
R-squared & 0.767 & 0.773 & 0.936 & 0.939 \\
\bottomrule
\end{tabular}
